Teaching VLMs to Localize Specific Objects from In-context Examples

Vision-Language Models (VLMs) have shown remarkable capabilities across diverse visual tasks, including image recognition, video understanding, and Visual Question Answering (VQA) when explicitly trained for these tasks. Despite these advances, we find that present-day VLMs (including the proprietary GPT-4o) lack a fundamental cognitive ability: learning to localize specific objects in a scene by taking into account the context. In this work, we focus on the task of few-shot personalized localization, where a model is given a small set of annotated images (in-context examples) -- each with a category label and bounding box -- and is tasked with localizing the same object type in a query image. Personalized localization can be particularly important in cases of ambiguity of several related objects that can respond to a text or an object that is hard to describe with words. To provoke personalized localization abilities in models, we present a data-centric solution that fine-tunes them using carefully curated data from video object tracking datasets. By leveraging sequences of frames tracking the same object across multiple shots, we simulate instruction-tuning dialogues that promote context awareness. To reinforce this, we introduce a novel regularization technique that replaces object labels with pseudo-names, ensuring the model relies on visual context rather than prior knowledge. Our method significantly enhances the few-shot localization performance of recent VLMs ranging from 7B to 72B in size, without sacrificing generalization, as demonstrated on several benchmarks tailored towards evaluating personalized localization abilities. This work is the first to explore and benchmark personalized few-shot localization for VLMs -- exposing critical weaknesses in present-day VLMs, and laying a foundation for future research in context-driven vision-language applications.

==> figures/ablation_mix.tex <==
\begin{figure}[t!]
    \centering
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/Ablation_Testing_Fake_Names_Average_IoU.pdf}
        \caption{\textbf{Focus on Context.} We report the mIoU (\%) on the ICL-LASOT test set by switching true category names with pseudo category names.}
        \label{fig:fake-names-data}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/llava_our.pdf}
        \caption{\textbf{Generalization of Finetuning.} We report the mIoU (\%) by fine-tuning \llava-OV~\cite{llava-ov} on our data mix and compare with baseline.}
        \label{fig:generalization-of-finetuning}
    \end{minipage}
\end{figure}



==> figures/localization_examples.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/localization copy v2.pdf} 
    \tabvcap
    \caption{\textbf{Examples of VLM localization.} The top row shows in-context shots, and the bottom row shows query images. Ground truth locations are marked in blue, and predicted locations in brown. (A) demonstrates successful localization without copying. (B) and (C) illustrate cases where the model replicates the in-context shot locations.}
    \label{fig:copying-shots}
    \figvb
    \vspace{-0.15cm}
\end{figure*}

% \begin{SCfigure*}[][t!]
%     \centering
%     \includegraphics[width=0.6\textwidth]{figures/localization copy v2.pdf} 
%     \caption{\textbf{Examples of VLM localization.} The top row shows in-context shots, and the bottom row shows query images. Ground truth locations are marked in blue, and predicted locations in brown. (A) demonstrates successful localization without copying. (B) and (C) illustrate cases where the model replicates the in-context shot locations.}
%     \label{fig:copying-shots}
% \end{SCfigure*}

==> method_CM/CM.tex <==
\subsection{How much does the model copy? Assessing Contextual Learning}


Excluding the GT\_Shot overlap in the IoU calculation serves as a metric to evaluate how much the model relies on visual context versus copying prior localizations. A high score here suggests that the model is using contextual information rather than memorized areas for localization.

\[
\text{IoU} = \frac{\max\left(0, A_{\text{Prediction} \cap \text{GT\_Query}} - A_{\text{Prediction} \cap \text{GT\_Shot}}\right)}{A_{\text{GT\_Query}} - A_{\text{GT\_Query} \cap \text{GT\_Shot}} + A_{\text{Prediction}} - \max\left(0, A_{\text{Prediction} \cap \text{GT\_Query}} - A_{\text{Prediction} \cap \text{GT\_Shot}}\right)}
\]

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/CM.png} 
    \caption{copy metric change name}
    \label{fig:CM}
\end{figure*}

Intersection over Union (IoU) Excluding Metric calculation for assessing contextual learning in localization models. In this formulation, \( A \) represents the area of different regions: \( A_{\text{GT\_Query}} \) is the area of the ground truth query box, \( A_{\text{GT\_Shot}} \) is the area of the ground truth shot box (a previously seen region), and \( A_{\text{Prediction}} \) is the area of the model's predicted box. The adjusted intersection excludes overlap with \( A_{\text{GT\_Shot}} \), allowing us to measure the IoU as an indicator of the model’s reliance on visual context over memorization.

==> tables/fake_ablation.tex <==
\begin{table*}[t!]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{10pt}
    \begin{tabular}{ c c c c c c}
        \toprule
        \textbf{Shots} & \textbf{Idefics3} & \textbf{\llava OV} & \textbf{Qwen-VL 7B} & \textbf{Our Real + Fake} & \textbf{Our Real}\\
                \midrule
          1 & 0.20 & 0.15 & 27.14 &\textbf{44.04}&33.77\\
         4 & 0.00 & 0.00 & 12.85 &\textbf{20.65}&11.84\\
         8 & 0.00 & 0.00 & 9.67 &\textbf{16.39}&9.7\\
        \bottomrule
    \end{tabular}
    \caption{Comparison of \%iou LASOT fake names}
    \label{tab:fake}
\end{table*}


==> tables/lasot-fake.tex <==
\begin{table*}[t!]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{10pt}
    \begin{tabular}{l c c c c c }
        \toprule
        \textbf{Shots} & \textbf{Idefics3} & \textbf{\llava OV} & \textbf{Qwen2-VL 7B} & \textbf{Ours Real + Fake} & \textbf{Ours Real}\\
        \midrule
          1 & 0.20 & 0.15 & 27.14 &\textbf{44.04}&33.77\\
         4 & 0.00 & 0.00 & 12.85 &\textbf{20.65}&11.84\\
         8 & 0.00 & 0.00 & 9.67 &\textbf{16.39}&9.7\\
        \bottomrule
    \end{tabular}
    \caption{Ablation for testing fake names, Comparison of ICL-LASOT Fake \% IoU}
    \label{tab:abl:Fake_LASOT}
\end{table*}

==> tables/quantity.tex <==
% \begin{table}[t!]
%     \centering
%     \renewcommand{\arraystretch}{1.2}
%     \setlength{\tabcolsep}{10pt}
%     \begin{tabular}{l c c c c c c }
%         \toprule
%         \textbf{Dataset} & \textbf{Amount}\\
%         \midrule
%         PDM & 1 & 976 \\
%         & 2 & 976 \\
%         \midrule
%         PerSeg & 1 & 40\\
%         & 2 & 40 \\
%         & 3 & 40\\
%         & 4 & 40 \\
%         \midrule
%         ICL-LASOT & 1 & 280 \\
%         & 4 & 280 \\
%         & 8 & 280 \\
%         \bottomrule
%     \end{tabular}
%     \caption{# of conversations in each test}
%     \label{tab:test_amount}
% \end{table}

\begin{table}[t!]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{10pt}
    \begin{tabular}{l c c }
        \toprule
        \textbf{Type} &\textbf{Dataset} & \textbf{\#Conversations}\\
        \midrule
        Train&LASOT  & 17,920 \\
        &TAO &  8,816\\
        &GOT & 56,010 \\
\midrule
        Test &PDM & 1,952 \\
        &PerSeg & 160 \\
        &ICL-LASOT & 840 \\
        \bottomrule
    \end{tabular}
    \caption{Amount of conversations for train and test}
    \label{tab:train_amount}
\end{table}

==> tables/semantically_coherent_data_vs_random.tex <==
\begin{table}[t!]
    \centering
    \begin{tabular}{lccc}
        \toprule
        Method & PerSeg & ICL-LASOT & PDM \\
        \midrule
        Arbitrary Video Sequences & 17.55 & 24.14 & 28.94 \\
        IPLoc Data Mix & 27.55 & 39.13 & 50.05 \\
        \bottomrule
    \end{tabular}
    \caption{Ablating the effect of sampling conversations from the same video (IPLoc) vs. arbitrary video sequences.}
    \label{tab:semantically_coherent_data}
\end{table}

==> tables/supp_data_mix.tex <==
\begin{table*}[h]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{6pt} % Adjust column spacing
    \begin{tabular}{l c c c c c}
        \toprule
        \textbf{Dataset} & \textbf{Shots} & \textbf{All Data} & \textbf{LASOT} & \textbf{GOT} & \textbf{TAO} \\
        \midrule
        PDM & 1 & \textbf{28.41} & 17.84 & 20.53 & 14.1 \\
         & 2 & \textbf{21.74} & 15.31 & 16.39 & 10.0 \\
                 \midrule

        PerSeg & 1 & \textbf{42.43} & 30.19 & 25.57 & 30.05 \\
        & 2 & \textbf{41.15} & 37.67 & 33.11 & 28.03 \\
        & 3 & \textbf{39.85} & 37.92 & 26.4 & 27.23 \\
        & 4 & 33.08 & \textbf{36.89} & 24.28 & 27.67 \\
                \midrule

        ICL-LASOT & 1 & \textbf{49.01} & 43.44 & 36.41 & 23.77 \\
         & 4 & 22.22 & \textbf{24.47} & 10.99 & 10.03 \\
         & 8 & 21.19 & \textbf{22.99} & 10.05 & 8.38 \\
                 % \midrule

        % ICL-LASOT fake & 1 & \textbf{44.04} & 41.37 & 27.05 & 16.95 \\
        %  & 4 & 20.65 & \textbf{21.19} & 8.85 & 8.77 \\
        %  & 8 & 16.39 & \textbf{21.3} & 9.34 & 8.1 \\
        \bottomrule
    \end{tabular}
    \caption{Ablation of data mixes}
    \label{tab:datamix_shots}
\end{table*}


==> tables/supp_llava_ov_train.tex <==
\begin{table*}[t!]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{10pt}
    \begin{tabular}{l c c c c}
        \toprule
        \textbf{Dataset} & \textbf{Shots} & \textbf{\llava OV} & \textbf{\llava OV trained} \\
        \midrule
        pdm & 1 & 1.27 & 0.43\\
        & 2 & 0.00 & 0.39\\
        \midrule
        perseg & 1 & 4.78 & 4.29\\
        & 2 & 0.00 & 2.99\\
        & 3 &  0.00 & 4.89 \\
        & 4 &  0.00 & 0.26\\
        \midrule
        LASOT & 1 & 1.10 &  1.86\\
        & 4 & 0.00 &  2.06\\
        & 8 & 0.00 & 0.46\\
        \bottomrule
    \end{tabular}
    \caption{Comparison of \% IoU LLaVa-OV with and without our training}
    \label{tab:miou_llava_ov_trained}
\end{table*}


==> tables/supp_prompt_big_models.tex <==
\begin{table*}[t!]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{l c | c c c c | c c c c}
        \toprule
        & & \multicolumn{4}{c|}{\textbf{InternVL2-76B}} & \multicolumn{4}{c}{\textbf{Qwen2-VL-72B}} \\
        \textbf{Dataset} & \textbf{Shots} & \textbf{Prompt 0} & \textbf{Prompt 1} & \textbf{Prompt 2} & \textbf{Prompt 3} & \textbf{Prompt 0} & \textbf{Prompt 1} & \textbf{Prompt 2} & \textbf{Prompt 3} \\
        \midrule
        pdm & 1 & 23.28 & 27.48 & 31.26 & 29.11 & 33.65 & 16.88 & 19.96 & 21.23 \\
        pdm & 2 & 14.20 & 21.87 & 28.67 & 20.85 & 32.37 & 12.97 & 13.11 & 12.29 \\
        \midrule
        perseg & 1 & 34.51 & 49.01 & 50.01 & 46.06 & 0.81 & 41.88 & 44.75 & 34.91 \\
        perseg & 2 & 24.18 & 41.16 & 51.46 & 42.30 & 0.90 & 35.47 & 28.19 & 28.68 \\
        perseg & 3 & 44.94 & 43.22 & 49.37 & 50.03 & 0.29 & 49.51 & 43.43 & 45.50 \\
        perseg & 4 & 36.57 & 34.63 & 45.70 & 42.34 & 1.26 & 39.96 & 37.36 & 31.04 \\
        \midrule
        LASOT & 1 & 40.67 & 42.47 & 47.68 & 46.07 & 4.82 & 42.66 & 43.14 & 43.01 \\
        LASOT & 2 & 23.21 & 45.61 & 42.90 & 43.76 & 0.40 & 38.05 & 40.04 & 37.65 \\
        LASOT & 4 & 31.72 & 39.71 & 38.90 & 38.86 & 1.63 & 33.54 & 31.29 & 31.38 \\
        LASOT & 8 & 21.65 & 21.74 & 27.21 & 29.18 & 0.76 & 31.17 & 22.81 & 27.23 \\
        \midrule
        Avg.  &   & 29.49 & 36.69 & 41.32 & 38.86 & 7.69 & 34.21 & 32.41 & 31.29 \\
        \bottomrule        
    \end{tabular}
    \caption{Comparison of \% IoU for "big" models according to the instruction}
    \label{tab:big_models_prompt}
\end{table*}


==> tables/supp_seedbench_ablation.tex <==
% \begin{table}[h!]
% \centering
% \begin{tabular}{|l|cccccccccc}
% \toprule
%  & Overall & Instance Attributes & Instance Identity & Instance Interaction & Instance Location & Instances Counting & Scene Understanding & Spatial Relation & Text Understanding & Visual Reasoning \\
% \midrule
% Baseline & 0.76 & 0.79 & 0.79 & 0.70 & 0.72 & 0.71 & 0.80 & 0.62 & 0.73 & 0.79 \\
% Ours (LORA FT)    & 0.75 & 0.78 & 0.78 & 0.70 & 0.70 & 0.70 & 0.80 & 0.58 & 0.71 & 0.79 \\
% Ours (Full FT)    0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.012 & 0.000 & 0.000 & 0.000 & 0.000 \\
% \bottomrule
% \end{tabular}
% \caption{Qwen SeedBench-Image variants results}
% \label{table:seedbench_results}
% \end{table}




\begin{table*}[h!]
\centering
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{10pt}
\begin{tabular}{lccc}
\toprule
\textbf{Metric} & \textbf{Qwen2-VL 7B} & \textbf{Ours Real + Fake (LORA FT)} & \textbf{Ours Real + Fake (Full FT)} \\
\toprule
Overall & 76.41 & 75.41 & 00.21 \\
\midrule
Instance Attributes & 78.77 & 77.84 & 00.02 \\
Instance Identity & 79.46 & 78.37 & 00.00 \\
Instance Interaction & 70.10 & 70.10 & 00.00 \\
Instance Location & 72.09 & 69.73 & 00.00 \\
Instances Counting & 71.15 & 69.76 & 01.19 \\
Scene Understanding & 79.61 & 79.70 & 00.00 \\
Spatial Relation & 61.64 & 58.30 & 00.00 \\
Text Understanding & 72.62 & 71.43 & 00.00 \\
Visual Reasoning & 79.46 & 79.15 & 00.00 \\
\bottomrule
\end{tabular}
\caption{Qwen SeedBench-Image variants results}
\label{table:abl:seedbench_results}
\end{table*}



==> tables/table_average.tex <==
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{6pt} % Adjust column spacing
    \begin{tabular}{l c c c c }
        \toprule
        \textbf{Model} & \textbf{PerSeg} & \textbf{PDM} & \textbf{ICL-LASOT} & \textbf{ICL-LASOT fake} \\
        \midrule
        QWEN2 VL 7B & 29.42 & 20.69 & 29.9 & 16.55 \\
        Our Real + Fake & \textbf{39.13} & 21.34 & \textbf{30.47} & \textbf{27.03} \\
        Our Real & 32.94 & \textbf{23.52} & 26.5 & 18.44 \\
        % Our full FT & 28.27 & 14.07 & 16.13 & 15.13 \\

        \bottomrule
    \end{tabular}
    \caption{Average miou (\%) across models and complex patterns}
    \label{tab:miou_average_across_patterns}
\end{table}

==> tables/table_full.tex <==
\begin{table*}[h]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{6pt} % Adjust column spacing
    \begin{tabular}{l c c c c c c c }
        \toprule
        \textbf{Model} & \textbf{1s perseg} & \textbf{1s tao} & \textbf{2s perseg} & \textbf{2s tao} & \textbf{3s perseg} & \textbf{4s perseg}  \\
        \midrule
        QWEN2 VL 7B & 34.21 & 20.55 & 30.22 & 23.69 & 35.09 & 18.16\\
        Our Real + Fake & 42.43 & 28.41 & \textbf{41.15} & 21.74 & \textbf{39.85} & \textbf{33.08} \\
        Our Real & \textbf{43.4} & \textbf{31.54} & 29.9 & \textbf{24.45} & 33.23 & 25.25 \\
        % Full FT & 35.32 & 19.89 & 29.89 & 14.21 & 25.57 & 22.3 & 8.11 \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of miou (\%) - Part 1}
    \label{tab:miou_comparison_part1}
\end{table*}

\begin{table*}[]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{6pt} % Adjust column spacing
    \resizebox{\textwidth}{!}{\begin{tabular}{l c c c c c c c }
        \toprule
        \textbf{Model} & \textbf{LASOT 1s} & \textbf{LASOT 4s} & \textbf{LASOT 8s} & \textbf{fake LASOT 1s} & \textbf{fake LASOT 4s} & \textbf{fake LASOT 8s} \\
        \midrule
        QWEN2 VL 7B & 46.69 & 21.89 & \textbf{21.12} & 27.14 & 12.85 & 9.67 \\
        Our Real + Fake & \textbf{49.01} & \textbf{22.22} & 20.19 & \textbf{44.04} & \textbf{20.65} & \textbf{16.39} \\
        Our Real & 46.98 & 16.99 & 15.52 & 33.77 & 11.84 & 9.7 \\
        % Full FT & 29.45 & 9.27 & 9.66 & 27.61 & 9.34 & 8.44 \\
        \bottomrule
    \end{tabular}}
    \caption{full Comparison of miou (\%)  - Part 2}
    \label{tab:miou_comparison_part2}
\end{table*}


==> tex/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We propose a data-centric approach to enhance the few-shot personalized object localization capabilities of modern VLMs. 
Our findings reveal that for VLMs to excel in this task, fine-tuning data must be semantically coherent, personalized, and designed to encourage reliance on contextual cues rather than pre-existing pre-training knowledge. 
To achieve this, we utilize multiple video object-tracking datasets and introduce innovative regularization schemes for constructing instruction-tuning conversations that provoke robust few-shot learning abilities in VLMs.
Through extensive evaluations and ablation studies across multiple benchmarks, we demonstrate the effectiveness of our proposed data and fine-tuning strategies. 
The results provide a fresh perspective on the impact of data-centric methods for advancing personalized localization capabilities in VLMs, offering valuable insights and a foundation for future work in this direction.


